VECA : A Toolkit for Building Virtual Environments to Train and Test Human-like Agents

Building human-like agent, which aims to learn and think like human intelligence, has long been an important research topic in AI. To train and test human-like agents, we need an environment that imposes the agent to rich multimodal perception and allows comprehensive interactions for the agent, while also easily extensible to develop custom tasks. However, existing approaches do not support comprehensive interaction with the environment or lack variety in modalities. Also, most of the approaches are difficult or even impossible to implement custom tasks. In this paper, we propose a novel VR-based toolkit, VECA, which enables building fruitful virtual environments to train and test human-like agents. In particular, VECA provides a humanoid agent and an environment manager, enabling the agent to receive rich human-like perception and perform comprehensive interactions. To motivate VECA, we also provide 24 interactive tasks, which represent (but are not limited to) four essential aspects in early human development: joint-level locomotion and control, understanding contexts of objects, multimodal learning, and multi-agent learning. To show the usefulness of VECA on training and testing human-like learning agents, we conduct experiments on VECA and show that users can build challenging tasks for engaging human-like algorithms, and the features supported by VECA are critical on training human-like agents.

==> Sections/0-AbstractNoHuman.tex <==


%The concept of \emph{cognitive agent}, capable of acting and interacting with an environment for cognitive development and learning, is receiving increasing attention as a way to overcome the limitations of deep learning algorithms. 

%The concept of \emph{human-like agent}, which aims to catch up the learning ability of human, is receiving increasing attention as a way to overcome the limitations of deep learning algorithms. 
%However, it is extremely challenging to develop such agents due to lack of tools to train and test them. 

With the dramatic improvement of machine learning algorithms, forming an environment where novel learning algorithms can show their full potential is receiving increasing attention in AI community. 
To maximize the potential of the agent, the environment must impose the agent to rich multimodal perception and allow comprehensive interactions for the agent. 
However, existing approaches (including datasets or virtual environments) does not support comprehensive interaction with the environment, or lack of modality.
In this light, we propose a novel VR-based toolkit, VECA, which enables to train and test emerging learning algorithms in a fruitful virtual environment. VECA provides: 1) richmultimodal perceptions, 2) comprehensive interaction capability with the environment 3) extensibility for various custom tasks, where developers can easily design challenging but also fruitful virtual environments.
To motivate and formulate VECA, we also provide a set of example environment and tasks which requires skills for the agent such as multimodal learning, multi-agent communication and cooperation, accurate control. 
To validate VECA, we conduct preliminary experiments on VECA and show that the features supported by VECA are critical to the agent's performance, even if the agent is trained using the same learning algorithm.

%In this paper, we propose a novel VR-based toolkit, VECA, which enables to train and test human-like agents in a virtual environment. In particular, VECA provides a virtual humanoid avatar with rich human-like perceptions and an environment for the agent to interact, with which development of human-like agents can be facilitated. 

%Our preliminary evaluation shows that the agent trained with rich perceptions can achieve higher learning performance for the task to kick a ball, while the agent with a single perception fails to learn certain interaction patterns thereby getting lower performance. 


==> Sections/1-Introduction_NoHuman.tex <==

\begin{document}

Recently machine learning methods have dramatically improved, outperforming previous state-of-the-art algorithms and even human intelligence in various domains such as image classification~\cite{ImagenetSurpass}, complex games such as Go or Starcraft 2~\cite{AlphaGo,Starcraft2}, which was expected to be impossible for decades.
%With the rapid improvement of machine learning algorithms, it has been argued the achievable performance of the agent (trained by machine learning algorithms) is bounded by the environment which is used to train and test the agent~\cite{AgentBounded}. 
With the rapid improvement of machine learning algorithms, it has been argued the achievable performance of learning algorithms is bounded by the environment which is used to train and test the agent~\cite{AgentBounded}. 
In this light, forming an environment where novel learning algorithms could show their full potential is receiving increasing attention in AI community.

%However, those are often in limited settings: . like human: embodied general agent. 
%There exists and disparency between current benchmarks and .
%In this light, researches about .  
%We need a training/testing bed to 

%More complicated, general tasks. 
%Next-generation agents would capability of 

%In short, current agent's performance could be limited its environmental settings: perception and action in specific.

%Recently deep learning methods have outperformed previous state-of-the-art algorithms and even human intelligence in various domains such as image classification~\cite{ImagenetSurpass}, complex games such as Go or Starcraft 2~\cite{AlphaGo,Starcraft2}. Despite those promising results, it has been argued that current deep learning methods are still apart from desired intelligence (i.e. general agents)~\cite{DeepLearningCritical}. 
%For instance, it requires a large amount of labeled data to train a model, which is highly costly and maybe impossible for certain tasks. Moreover, trained models are hard to interpret since it works as an black-box model. Furthermore, the structure of the model and its training processes are highly task-specific. A model built for a particular task does not apply even to similar tasks or the same task with different settings~\cite{Schema}. 
%Due to aforementioned limitations, current deep learning agents struggle in tasks such as few-shot learning where human intelligence shines. 

%and has reported promising results, such as human-level accuracy in certain types of classification/prediction tasks\cite{DeepLearning}. However, despite those achievements of deep learning, there has been reported that deep learning has some fundamental problems. 

%One of the problems of deep learning is interpretability\cite{Interpret}. Deep learning is mainly black-box statistical learning with datasets. It requires a large amount of labeled data, which is costly or maybe impossible for certain tasks. Moreover, it makes the agent hard to deal with corner cases because the passively collected dataset can't show all of the massive diversity of the task. Furthermore, it is hard to check whether the agent is 'cheating' or not, since deep learning models is hard to interpret.

%Another problem of deep learning is task-dependence. Currently, the model structure and training process of the agent is task-specific. For example, knowledge or useful features gained by models for computer vision tasks are not applied in natural language processing tasks, which include various visual concepts. Although transfer learning\cite{transfer1, transfer2} and multi-task learning\cite{multi1, multi2} tackles some of the problems with shared weights, those works aim to learn pre-defined tasks with the same type of data. Since real-world problems consist of multiple and unexpectable tasks, training the model one by one for all tasks is impossible. 

%One of the promising direction to overcome such limitations is to bring inspiration from the well-known interpretable and data-efficient general intelligence: a human intelligence. Although there is no need to, and even if should not, duplicate human intelligence (which is error-prone and imperfect), still human intelligence is an attractive target intelligence to learn and get inspiration about how to learn~\cite{DeepLearningCritical}. Accordingly, discussions and works about building human-like agents~\cite{BuildingMachine,HumanLikeAgent} have been made.

%However, the agent's performance also bounds from the environment (independent to the algorithm). For example, the agent may have a hard time or unable to learn concepts such as noisy/quiet and rough/smooth  without audio and tactile perception. Human intelligence also benefits from , To next-generation agents, we need 

To maximize the capability of the learning machine and fully expose its potential, the machine must be imposed to rich multimodal perception and able to interact with the environment. Prior works in developmental psychology suggest that human intelligence learns by experience~\cite{Gibson, Piaget}, which consists of collecting rich multimodal perception from the environment~\cite{ObjectPerception,PerCog} and actively interacting~\cite{Active1,LearningPlay} with it.
%For instance, developmental psychologists have studied that general understanding of objects develops in an early stage of the toddler without any supervision, by receiving multimodal feedback during interaction on objects such as mouthing, chewing, and rotating\cite{Gibson,Piaget}. 
Similar to human intelligence, it has been also argued that artificial intelligence could benefit from multimodal~\cite{de2017guesswhat,ngiam2011multimodal} and interactive~\cite{caselles2019symmetry,hermann2017grounded} learning. %To build an agent learn like human, it is crucial to provide rich multimodal perception (such as audio, tactile) and interactions for the agent.

% In short, human intelligence learns by experience; by collecting \textbf{rich sensory information} from an environment and \textbf{actively interacting} with it.

%In this point, how human intelligence learn general tasks in a data-efficient way remains as a question. Although there are multiple times of general intelligence, 
%On top of that, which is also reported by various works from development science. 
%In short, human intelligence agent learns by experience; by collecting \textbf{rich sensory information} from an environment and \textbf{actively interacting} with it.

%Action and perception defines an agent.

%With lack of perception, misunderstanding can occur even for human intelligence. 

%We suggest that training and testing those agent requires at least major features of human perception.

%We can't expect the agent to gain general knowledge while playing atari.
%A promising direction to overcome such limitations of deep learning is developing \textit{cognitive agents} (interchangeably with cognitive models or algorithms) \cite{Cognitive} that imitate human-like perceptions and thought process. Reflecting how human learn, cognitive agent aims at learning \emph{generic tasks} by continuously \emph{observing environments with various sensory perceptions} and \emph{interacting with environments}. For instance, a cognitive agent learns "how to recognize a dog" using multi-modal perceptions (e.g., visual, auditory, and tactile perceptions) obtained while interacting with dogs (e.g. observing different appearance of dogs while playing), whereas current deep learning algorithms learn the same by building a statistical model with a large pre-collected dog images. 

%In specific, cognitive agents 'understands' the perception while statistic models 'extract task-specific features from the perception. For example, if a cognitive agent sees a tree image, it classifies the image as a tree based on a general understanding of tree (e.g. green leaves connected with brown thick stem). However, image classification model trained with deep learning will extract features only relevant to classification. If the number of green and brown pixels is sufficient to classify tree images as a tree, the model might learn as 'green + brown is a tree'. 

%aims to understand and gain knowledge from perceptions by interpreting their perceptions with their experiences\cite{Cognitive}. Because cognitive agents aim to interpret its perception, it solves the problem of interpretability. Also, it solves the problem of task-dependence because cognitive agents try to understand and gain general knowledge, rather than just extracting task-relevant features from perceptions as deep learning.  

%One of the approaches to solve this problem is to train a \textit{cognitive} agent. Cognitive agent aims to understand and gain knowledge from perceptions by interpreting their perceptions with their experiences\cite{Cognitive}. Because cognitive agents aim to interpret its perception, it solves the problem of interpretability. Also, it solves the problem of task-dependence because cognitive agents try to understand and gain general knowledge, rather than just extracting task-relevant features from perceptions as deep learning.

%Because of its characteristics, it is challenging to develop new human-inspired agents due to lacking tools (environments) to train and test them. 
However, providing rich multimodal perception and interactions is not an easy job. An intuitive way would be to develop a robot with an actionable body and sensors, but building such robot is often highly costly. Also, it is difficult to test premature agents that may break robot hardware. Moreover, speed of the training process is limited to the real-time scale since the robot has to perceive and interact in the real world. Another promising approach is to train the agent in a virtual environment. Existing environments such as game environments for reinforcement learning \cite{ALE,OpenAIUniverse,DeepMindLab,Malmo,VizDoom,Arena}, however, oversimplifies dynamics and perceptions of game avatars, which makes them inappropriate for developing human-like agents. There have been recent efforts to simulate realistic indoor environments \cite{GibsonEnv,AI2-THOR,HoME,House3D,MINOS}, but they do not support active interactions or lack of rich multi-modal perceptions. 

%However, it is challenging to develop new human-inspired agents due to lacking tools (environments) to train and test them. The key challenge lies in that human intelligence learns by experience; by collecting \textbf{rich multi-modal information} from an environment and \textbf{actively interacting} with it. An intuitive way would be to develop a robot with an actionable body and sensors, but building such a human-like robot is highly costly. Also, it is difficult to test premature agents that may break robot hardware. Moreover, accelerating the training process is not straightforward since the robot has to perceive and interact in the real world. Another promising approach is to train the agent in a virtual environment. Existing environments such as game environments for reinforcement learning \cite{ALE, OpenAIUniverse, DeepMindLab, Malmo, VizDoom, Arena}, however, oversimplifies dynamics and perceptions of game avatars, which makes them inappropriate for developing cognitive agents. There have been recent efforts to simulate realistic indoor environments \cite{Gibson, AI2-THOR, HoME, House3D, MINOS}, but they do not support active interactions or lack of rich multi-modal perceptions. 

%Despite its potential, it is challenging to develop new cognitive agents due to lacking tools to train and test them. The key challenge lies in that a cognitive agent has to learn by experience; by collecting \textbf{rich sensory information} from an environment and \textbf{actively interacting} with it. An intuitive way would be to develop a robot with an actionable body and sensors. However, building such a human-like robot is highly costly. Also, it is difficult to test premature agents that may break robot hardware. Moreover, accelerating the training process is not straightforward since the robot has to perceive and interact in the real world. Another promising approach is to train the agent in a virtual environment. Existing environments such as game environments for reinforcement learning \cite{ALE, OpenAIUniverse, DeepMindLab, Malmo, VizDoom, Arena}, however, oversimplifies dynamics and perceptions of game avatars, which makes them inappropriate for developing cognitive agents. There have been recent efforts to simulate realistic indoor environments \cite{Gibson, AI2-THOR, HoME, House3D, MINOS}. However, they do not support active interactions or lack of multi-modal perceptions. 

%Then what does cognitive agent need? Since cognitive agent has to understand the perception and learn in a self-directed way e.g. by experience without passive datasets, they need \textbf{rich sensory information} and \textbf{various interaction} with the environment. 

%To provide rich sensory inputs, it is important to choose how to represent the senses. There are various ways to define the senses. For instance, vision can be modeled as a first-person view RGB binocular vision similar to humans but also can be modeled as a panorama of depth map using radar. One of the promising ways is to model human perception. First, there are fields in which we need human perception. For example, agents like to require a deep comprehension of humans, and it can't be learned without human perception. Second, it is 'confirmed' that this representation is good for massive kinds of tasks. Since we want the agents to help our works, the most intuitive and plausible representation would be to mimic our perception. 

%Then where can we train those cognitive agents? The most promising way would be to train them in the real world. However, it will require a robot with lots of sensors, which is fragile and expensive. Moreover, the time scale of the training process would be restricted to real-time. Thus, the most reasonable way would be to train the agent in a virtual environment. However, existing environments lack in this purpose. Most of the environments, such as game environments\cite{Game1, Game2}, oversimplifies its dynamics and perception. Although there are environments that aim to give real-like perception\cite{Gibson,realistic2,realistic4}, those environments are static and hard to integrate those environments to custom tasks.
 
%자랑. 왜 VECA 가 cognitive agent를 잘 train 할수 있나..

In this light, we propose a novel VR-driven toolkit, VECA, which enables to train and test emerging learning algorithms in a virtual environment. VECA provides several essential features where the user could design challenging environments for task-hungry learning algorithms: 1) rich multimodal perceptions, 2) comprehensive interaction capability with the environment 3) extensibility for various custom tasks. Using VECA, developers can easily design challenging but also fruitful environments, which could broaden the scope of learning algorithms. 


%Using VECA, developers can easily create a custom environment where an agent can take sensory inputs, learn cognition in a self-directed manner, and perform necessary actions to collect rich sensory data or improve cognitive capability. 

%In this light, we propose a novel VR-driven toolkit, VECA, which enables to train and test emerging human-like agents in a virtual environment. VECA provides several essential features to train human-like agents: 1) rich multimodal perceptions, 2) comprehensive interaction capability with the environment 3) extensibility for various custom tasks. 
%We choose to use human-like perceptions because human perception is rich enough to reach human-level intelligence, and also we are targeting human-like agents.
%Using VECA, developers can easily create a custom environment where an agent can take sensory inputs, learn cognition in a self-directed manner, and perform necessary actions to collect rich sensory data or improve cognitive capability. 

%VECA detail
More specifically, VECA is implemented over the Unity engine and provides example virtual rooms, interactable objects, and environments for certain tasks. To provide rich multimodal perception and comprehensive interaction capability, we choosed the agent to be a humanoid. VECA provides a humanoid avatar and simulate various human-like perceptions such as binocular vision, spatialized binaural audio, tactile sense, and proprioception. Also, it enables the agent to interact with objects based on physics or pre-defined animations. Users can easily use VECA by simply specifying which sensory data to collect and providing agents to develop cognitions and perform specific actions given sensory input. Our evaluation shows the feasibility and usefulness of VECA with a set of example tasks. 

%VECA is implemented over the Unity engine, and provide realistic dynamics and easily customizable environments. 

%Also, we provide a framework that contains useful libraries about perception. 

%VECA evaluation
%To validate VECA, we conducted a preliminary study with a set of cognitive tasks(cross-modal learning, active data generation). We don't aim to propose novel structure or algorithms for cognitive agents: this task shows that VECA gives enough information to train cognitive agents. 

The contribution of this work can be summarized as follows:

\begin{itemize}
\item {We propose a novel VR-based toolkit named VECA to train and test next-generation learning algorithms in a virtual environment. VECA is the very first tool that provides rich human-like multimodal perceptions and interaction capability with a human avatar, which will serve as the cornerstone to develop environments for innovative models and algorithms. }

%\item {We enable VECA to support human-like perceptions with a suite of simulation techniques. }

\item {To motivate and formulate VECA, we provide a set of example environments and tasks (e.g. kicking a ball, grab an object, learn to cooperate using auditory perception, etc.) which could be directly used or modified.} %Please note that VECA is a toolkit, which allows the users to easily create a new learning environment suitable for novel human-like agents.}

\item {We conduct preliminary experiments on VECA and show that features of VECA are important for training and testing learning algorithms.
%Specifically, the agent achieves the best learning performance when it uses multiple sensory inputs and interacts with objects with a good exploration strategy.
For instance, we conduct an ablation study on the quality of perception of the agent, and show that the features of perceptions provided by VECA is critical to the agent’s performance.
}
%In our study, the agent achieved the best learning performance when it uses multiple sensory inputs and interacts with objects with good strategy. This shows that rich sensory inputs and interactions, which are the unique features of VECA, are important in building a cognitive agent.}
\end{itemize}

\end{document}

